Hybrid Batch Attacks: Finding Black-box Adversarial Examples with Limited Queries

We study adversarial examples in a black-box setting where the adversary only has API access to the target model and each query is expensive. Prior work on black-box adversarial examples follows one of two main strategies: (1) transfer attacks use white-box attacks on local models to find candidate adversarial examples that transfer to the target model, and (2) optimization-based attacks use queries to the target model and apply optimization techniques to search for adversarial examples. We propose hybrid attacks that combine both strategies, using candidate adversarial examples from local models as starting points for optimization-based attacks and using labels learned in optimization-based attacks to tune local models for finding transfer candidates. We empirically demonstrate on the MNIST, CIFAR10, and ImageNet datasets that our hybrid attack strategy reduces cost and improves success rates. We also introduce a seed prioritization strategy which enables attackers to focus their resources on the most promising seeds. Combining hybrid attacks with our seed prioritization strategy enables batch attacks that can reliably find adversarial examples with only a handful of queries.

==> 04_table4-cut.tex <==
\begin{table}[]
%%! please don't scale tables unless absolutely necessary \scalebox{0.92}
{
\centering
\def\arraystretch{1.2}
\begin{tabular}{ccc}
\toprule
& \multicolumn{2}{c}{Local Model Ensemble} \\
Target Model & \model{NA}, \model{NB}, \model{NC} & \model{R-DenseNet}, \model{R-ResNet} \\ \hline
Normal & \textbf{63.3\%} & 17.0\% \\ %\hline
Robust & 10.1\% & \textbf{40.8\%} \\ \hline
\end{tabular}
}
\caption{Direct transfer rates for candidate adversarial examples found using different local model ensembles. The Normal model is \dnote{...}, the Robust model is \dnote{...} (are these just the ones described earlier?) If only results for CIFAR10, include in caption, but makes more sense to include both tasks here.
\dnote{does NA-NC means \model{NA}, \model{NB}, and \model{NC}?
}}
\label{tab:cifar10_trans_local_model_comp}
%%! \vspace{-1em} please don't put in spacing tricks like this
\end{table}




==> 09_more_results.tex <==
\section{Fine-tuning Local Model with Label by-Products}
\label{appex_sec:loc_model_tune}
In this section, we first provide results of fine-tuning local models based on the label by-products from baseline gradient attacks (i.e., attack starts from the original seed) in Table \ref{tab:hypo_2_validate}. 

%In Table \ref{appex_tab:label_prod_size_1} and Table \ref{appex_tab:label_prod_size_2}, we provide the results of total number of label by-products produced during the attack process of baseline gradient attack and the hybrid attack.

\begin{table*}[]
\centering
\begingroup
\setlength{\tabcolsep}{0.45em}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Dataset & \multicolumn{4}{c|}{MNIST} & \multicolumn{4}{c|}{CIFAR10} \\ \hline
Target Model Type & \multicolumn{2}{c|}{Normal} & \multicolumn{2}{c|}{Robust} & \multicolumn{2}{c|}{Normal} & \multicolumn{2}{c|}{Robust} \\ \hline
Gradient Attack & AutoZOOM & NES & AutoZOOM & NES & AutoZOOM & NES & AutoZOOM & NES \\ \hline
Label By-Product Size & 747,500 & 50,960 & 1,897,500 & 77,720 & 565,500 & 21,760 & 850,000 & 61,700 \\ \hline
\end{tabular}
\caption{Label By-product size of Experiment (Baseline + H2): \footnotesize{when the label by-product size exceeds a certain threshold (60,000 for MNIST and 50,000 for CIFAR10), random sampling is performed to limit the size of label by-products.}}
\label{appex_tab:label_prod_size_1}
\endgroup
\end{table*}

\begin{table*}[]
\centering
\begingroup
\setlength{\tabcolsep}{0.45em}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Dataset & \multicolumn{4}{c|}{MNIST} & \multicolumn{4}{c|}{CIFAR10} \\ \hline
Target Model Type & \multicolumn{2}{c|}{Normal} & \multicolumn{2}{c|}{Robust} & \multicolumn{2}{c|}{Normal} & \multicolumn{2}{c|}{Robust} \\ \hline
Gradient Attack & AutoZOOM & NES & AutoZOOM & NES & AutoZOOM & NES & AutoZOOM & NES \\ \hline
Label By-Product Size & 147,000 & 17,980 & 1,885,000 & 74,475 & 136,000 & 6,940 & 824,500 & 54,768 \\ \hline
\end{tabular}
\caption{Label By-product size of Experiment (Baseline + H1 + H2)} 
\label{appex_tab:label_prod_size_2}
\endgroup
\end{table*}

\section{Exploration of Other Local Information based Metrics}
\label{sec:candi_sel}
In this section, we show the exploration of other local information based metric in prioritizing seeds in the first stage of the second stage strategy, in addition to the PGD-Steps mentioned in Section \ref{sec:seed_prior_first_stage}. 

\subsection{Prioritizing based on the Gap in Prediction Confidence}
We observe that directly transferable seeds tend to have higher confidence gap compared to the non-transferable examples. Therefore, we prioritize seeds with higher confidence gap. The confidence gap is defined by slightly modifying the high confidence CW loss in \cite{carlini2017towards} \footnote{we just remove the term $\kappa$ in the original high confidence CW loss} with respect to the local models. Specifically, for targeted attacks, we define the confidence gap as $l(\mathbf{x},t) = \{\text{max}_{i \neq t} [Z(\mathbf{x})]_{i}-Z(\mathbf{x})_{t}\}$ where $Z(\mathbf{x})$ denotes the logit score distribution (prediction from logit layer) of a seed. Thus, $Z(\mathbf{x})_{i}$ is the model's prediction of the logit score that $\mathbf{x}$ is in class $i$. Similarly, for the untargeted attack with ground-truth label $y$, the confidence gap is defined as $l(\mathbf{x},y) = \{Z(\mathbf{x})_{y} - \text{max}_{i\neq y}[Z(\mathbf{x})]_{i}\}$. We further observe that, it gives better prioritization performance when we first group the seeds based on number of local models been successfully attacked and then sort seeds in each group based on the confidence gap value. For example, when we have $K$ local models, we create $K+1$ groups for the seeds and group $k$ denotes successfully attacking $k~(k = 0,1,...,K)$ local models. Seeds in group $K$ is considered first, group $K-1$ comes second, similar logic applies for other groups with group $0$ being considered last. For each group, seeds are then ordered based on their confidence value gap. When there are multiple models in the local ensemble, the value of the confidence gap is ambiguous as each individual local NCan produce a unique confidence gap value with respect to the same local AE. Therefore, we consider three different values of confidence gap: \textit{Max-Gap} (maximum of all confidence gap values of local models), \textit{Min-Gap} (minimum of all confidence gap values of local models) and \textit{Ave-Gap} (average of all confidence gap values of local models). 

\subsection{Evaluation of Different Seed Prioritization Metrics}
\label{appex_sec:explore_loc_metrics}
In this section, we show the performance of different local model information based prioritization metrics, including the PGD-Step introduced in Section \ref{sec:seed_prior_first_stage}. We show effectiveness of seed prioritization strategies by the increased candidate transfer rate when candidates are carefully selected from the prioritized seeds, compared to random selection of candidates. 
%Next, we show effectiveness of transfer check over exhaustive execution in the first stage by showing more number of AEs found within same amount of query resources \footnote{Second stage of the two-stage strategy is exhaustive execution of gradient attack on remaining non-transfers. Therefore, showing effectiveness of transfer check in the first stage can validate the overall effectiveness of two-stage strategy over exhaustive execution of gradient attacks.}.
We reason about the improved transferability from the high candidate transfer rate when candidates are carefully selected from the prioritized seeds.
%and 2) increased number of AEs found with prioritization strategy in the first stage. We adopt the same datasets, models and attack strategies as in Section \ref{sec:hybrid_evaluation} for evaluation.

\shortsection{Improved Candidate Transfer Rate with Seed Prioritization} 
We show in Section \ref{subsec:valid_hypo} that when the candidates are selected as AEs succeed against all local models, candidate transfer rate can be much higher than the overall transfer rate and it is beneficial for attackers in batch setting as only the candidates are queried and can lead to significant portion of direct transfers. In this section, we also reason about the transferability from the point of candidate rate and candidate transfer rate by exploring more diverse candidate selection criteria. To be more specific, we first prioritize seeds based on the local information (i.e., confidence gap or PGD-Steps in Section \ref{sec:seed_prior_first_stage}). The prioritized seeds can provide different candidate rates and the corresponding candidate transfer rates: consider the case of a candidate pool with $n$ number of seeds, once sorted, the first $i~(1\leq i \leq n)$ images in the sorted list denotes the case where candidate rate is $i/n$. Direct transfer rate is then measured on the first $i$ images. Checking the first $i$ images cost exactly $i$ queries and therefore, high candidate transfer rate leads to more number of AEs found within the $i$ queries. We compare our seed prioritization strategies to the optimal and random candidate selection strategies: 

\begin{itemize}
\item \emph{Ideal Candidate Selection} -- this is an upper bound for the candidate transfer rate. This assumes attacker has access to a candidate selection oracle, which is able to prioritize all directly transferable seeds within the candidate slots \footnote{For example, when the overall transfer rate is 50\%, when the candidate rate is 50\%, the ideal candidate transfer rate is 100\% as all directly transferable samples are selected as candidates.}. Such an oracle is an ideal case and not achievable as attacker does not have prior knowledge on which seed directly transfers. 

\item \emph{Random Candidate Selection} -- This is the baseline strategy, where the candidates are selected at random from the total seeds. The candidate transfer rate will be equal to the overall transfer rate because of the random ordering of images. 
\end{itemize}

To eliminate the impact of random noise when the candidate rates are low, we repeat the experiments with 5 independent runs (in each run, 1000 examples with 100 seeds from each class are selected). For simplicity of presentation, we only present results on robust CIFAR10 models. Since there are normal and robust local models, we present results of the cases of all normal and all robust local ensembles \footnote{We also tested with mixture of normal and robust models, and similar patterns are observed. Due to space limitation, we omit all other local ensemble types.}. 

For all cases, we observe that when the candidates rates are low with respect to the sorted images, direct transfer rates of candidates can be much higher than the transfer rate of randomly selected candidates (i.e., overall transfer rate). In addition, we also observe that, there are some significant gaps between ideal transferability and the transferability of prioritized seeds. In Figure \ref{fig:candi_selection_robust_untar_cifar10}, we show transfer rate results of untargeted attacks on robust CIFAR10 model. Figure \ref{fig:candi_selection_robust_untar_cifar10_dense_resnet_vgg} denotes the case of local ensemble of all normal models. When the candidate rate is 0.1\%, the direct transfer rate of PGD-Steps is 80\% while the overall transfer rate (alternatively, the candidate transfer rate of randomly selected candidates) is only 9.9\%, a more than 8 times improvement. Similarly, when the local ensembles are all robust models, with Min-Gap or PGD-Step and with 5\% candidate rate, the candidate transfer rate can be improved to 83.2\% while the overall transfer rate is only 40.1\%, a more than 2 times improvement. For standard CIFAR10 DenseNet target model, with all robust local ensembles, candidate transfer rate can be improved to 80\% when candidate rate is 0.1\% (see the lines of Max-Gap and Min-Gap) while the overall transfer rate is only 18\%. 

As a conclusion, we observe that, when candidates are carefully selected based on the seed prioritization, attackers can have much higher transfer rates compared to the candidate transfer rate of randomly selected candidates. In addition, for different pairs of target and local models, the best performing metric typically differs, but the performance variation of different metrics are not very big.

    \begin{figure*}[ht]
        \centering
        \begin{subfigure}[b]{0.457\textwidth}
            \centering
            \includegraphics[width=\textwidth,height=5.5cm]{imgs/candidate_selection/cifar10-madry/untargeted/modelB_D_E.png}
            \caption[]%
            {Local Model: NA NB NC}    
            \label{fig:candi_selection_robust_untar_cifar10_b_d_e}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.457\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=5.5cm]{imgs/candidate_selection/cifar10-madry/untargeted/densenet_resnet.png}
            \caption[]%
            {Local Model: Adv-ResNet Adv-ResNet}    
            \label{fig:candi_selection_robust_untar_cifar10_dense_resnet_vgg}
        \end{subfigure}
        \vskip\baselineskip
        \caption[]
         {Untargeted adversarial examples on Madry robust CIFAR10 model: candidate rate and candidate transfer rate. {\em Ideal} denotes the case where attacker has oracle knowledge of transferability of each seed.} 
        \label{fig:candi_selection_robust_untar_cifar10}
    \end{figure*}

    \begin{figure*}[ht]
        \centering
        \begin{subfigure}[b]{0.457\textwidth}
            \centering
            \includegraphics[width=\textwidth,height=5.5cm]{imgs/candidate_selection/cifar10-densenet/modelB_D_E.png}
            \caption[]%
            {Local Model: NA NB NC}    
            \label{fig:candi_selection_norm_tar_cifar10_b_d_e}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.457\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=5.5cm]{imgs/candidate_selection/cifar10-densenet/densenet_resnet.png}
            \caption[]%
            {Local Model: Adv-DenseNet Adv-ResNet}    
            \label{fig:candi_selection_norm_tar_cifar10_dense_resnet_vgg}
        \end{subfigure}
        \vskip\baselineskip
        \caption[]
         {Targeted adversarial examples on standard CIFAR10 DenseNet model: candidate rate and candidate transfer rate. {\em Ideal} denotes the case where attacker has oracle knowledge of transferability of each seed.} 
        \label{fig:candi_selection_norm_tar_cifar10}
    \end{figure*}

\section{Seed Prioritization on Baseline Attacks}\label{appex_sec:h4_baseline}
In this section, we provide comprehensive evaluation of the impact of target loss based prioritization strategy on the baseline attack. Details are shown in Figure \ref{fig:h4_test_nes} and Figure \ref{fig:h4_test_autozoom}. In most cases, the greedy seed prioritization strategy works much better than random scheduling and has closer performance to retroactive optimal case. Only on ImageNet model, we observe that performance gain over random scheduling is not significant (see Figure \ref{fig:h4_test_nes_imagenet} and Figure \ref{fig:h4_test_autozoom_imagenet}). Discussion about this issue can be referred to the end of Section \ref{sec:prior_metric_eval}. 
%We also provide more detailed quantitative information of the prioritization of baseline attacks with the target loss value (Table \ref{appex_tab:baseline_prior}). 

    \begin{figure*}[ht]
        \centering
        \begin{subfigure}[b]{0.33\textwidth}
            \centering
            \includegraphics[width=\textwidth, height=4.5cm]{imgs/revision_imgs/h4_test/mnist/robust_mnist_nes.png}
            \caption[]%
            {Robust MNIST Model}    
            %\label{fig:h4_test_cifar10_robust_nes}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}
            \centering
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/h4_test/mnist/normal_mnist_nes.png}
            \caption[]%
            {Standard MNIST Model}    
            %\label{fig:h4_test_cifar10_robust_nes}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}
            \centering
            \includegraphics[width=\textwidth, height=4.5cm]{imgs/revision_imgs/h4_test/cifar10/cifar10_robust_nes.png}
            \caption[]%
            {Robust CIFAR10 Model}    
            %\label{fig:h4_test_cifar10_robust_nes}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.35\textwidth}
            \centering
            \includegraphics[width=\textwidth]{imgs/revision_imgs/h4_test/cifar10/cifar10_normal_nes.png}
            \caption[]%
            {Standard CIFAR10 Model}    
            \label{fig:h4_test_cifar10_robust_nes}
        \end{subfigure}
        \hspace{0.2in}
        \begin{subfigure}[b]{0.35\textwidth}
            \centering
            \includegraphics[width=\textwidth]{imgs/revision_imgs/h4_test/imagenet/imagenet_nes.png}
            \caption[]%
            {Standard ImageNet Model}    
            \label{fig:h4_test_nes_imagenet}
        \end{subfigure}
        % \hfill
        % \vskip\baselineskip
        % \quad
        \caption[]
        {Impact of Seed Prioritization on Baseline Strategy based on NES \footnotesize{x-axis denotes the query budget available for the attacker,y-axis denotes the number of AEs found within the provided budget.}} 
        \label{fig:h4_test_nes}
    \end{figure*}

    \begin{figure*}[ht]
        \centering
        \begin{subfigure}[b]{0.33\textwidth}
            \centering
            \includegraphics[width=\textwidth, height=4.5cm]{imgs/revision_imgs/h4_test/mnist/robust_mnist_autozoom.png}
            \caption[]%
            {Robust MNIST Model}    
            %\label{fig:h4_test_cifar10_robust_nes}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}
            \centering
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/h4_test/mnist/normal_mnist_autozoom.png}
            \caption[]%
            {Standard MNIST Model}    
            %\label{fig:h4_test_cifar10_robust_nes}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}
            \centering
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/h4_test/cifar10/cifar10_robust_autozoom.png}
            \caption[]%
            {Robust CIFAR10 Model}    
            %\label{fig:h4_test_cifar10_robust_nes}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.35\textwidth}
            \centering
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/h4_test/cifar10/cifar10_normal_autozoom.png}
            \caption[]%
            {Standard CIFAR10 Model}    
            %\label{fig:h4_test_cifar10_robust_nes}
        \end{subfigure}
        \hspace{0.2in}
        \begin{subfigure}[b]{0.35\textwidth}
            \centering
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/h4_test/imagenet/imagenet_autozoom.png}
            \caption[]%
            {Standard ImageNet Model}    
            \label{fig:h4_test_autozoom_imagenet}
        \end{subfigure}
        \caption[]
        {Impact of Seed Prioritization on Baseline Strategy based on AutoZOOM} 
        \label{fig:h4_test_autozoom}
    \end{figure*}
    
    
\section{Query Visualization of Starting from Local AEs and Original Seeds}
\label{appex_sec:per_example_compare}
In order to give a more intuitive idea about the difference of starting from the original seed and the local AE for each seed (average statistical information is provided in Table \ref{tab:hypo_loc_adv_sample}), we plot the per seed query distribution that starts from the original seed and local AE. Results are shown in Figure \ref{fig:adv_orig_query_nes} and Figure \ref{fig:adv_orig_query_autozoom}, corresponding to NES and AutoZOOM attacks separately. Note that, against attacks against standard MNIST, CIFAR10 and ImageNet models are targeted attacks with least likely class as the target class. For robust MNIST and robust CIFAR10 models, the attacks are untargeted attacks. To clarify, images in each figure is sorted based on the query number of starting from the original seed. 


    \begin{figure*}[ht]
        \centering
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth]{imgs/revision_imgs/adv_orig_query_dsitribution/mnist/normal_mnist_nes.png}
            \caption[]%
            {Target Model: Standard MNIST\newline}    
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}
            \centering
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/adv_orig_query_dsitribution/mnist/robust_mnist_nes.png}
            \caption[]%
            {Target Model: Robust MNIST\newline}    
            %\label{fig:adv_orig_query_normal_cifar10}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/adv_orig_query_dsitribution/cifar10/normal_cifar10_normal_local_nes.png}
            \caption[]%
            {Target Model: Standard CIFAR10, Local Model: NA, NB, NC}
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/adv_orig_query_dsitribution/cifar10/normal_cifar10_robust_local_nes.png}
            \caption[]%
            {Target Model: Standard CIFAR10, Local Model: R-ResN, R-DenseN}    
            
        \end{subfigure}
        \hfill
                \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/adv_orig_query_dsitribution/cifar10/robust_cifar10_normal_local_nes.png}
            \caption[]%
            {Target Model: Robust CIFAR10, Local Model: NA, NB, NC} 
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/adv_orig_query_dsitribution/cifar10/robust_cifar10_robust_local_nes.png}
            \caption[]%
            {Target Model: Robust CIFAR10, Local Model: R-ResN, R-DenseN}    
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/adv_orig_query_dsitribution/imagenet/nes.png}
            \caption[]%
            {Target Model: Standard ImageNet}    
            %
        \end{subfigure}
        \vskip\baselineskip
        \quad
        \caption[]
        {NES Attack: Query Distribution Comparison of Starting from Local AE and Original Seed. \footnotesize{Local models for generating local AEs are all normal models. Images are sorted by their corresponding query number of starting from the original seed. Images at 4,000 query of MNIST and CIFAR10 are failed adversarial examples. Images at query 10,000 fails for ImageNet. Attacks on robust MNIST and CIFAR10 models are untargeted attacks and the rest are targeted attacks with least likely class as the target class.}} 
        \label{fig:adv_orig_query_nes}
    \end{figure*}


    \begin{figure*}[ht]
        \centering
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/adv_orig_query_dsitribution/mnist/normal_mnist_autozoom.png}
            \caption[]%
            {Target Model: Standard MNIST\newline}    
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}
            \centering
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/adv_orig_query_dsitribution/mnist/robust_mnist_autozoom.png}
            \caption[]%
            {Target Model: Robust MNIST\newline}    
            %\label{fig:adv_orig_query_normal_cifar10}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/adv_orig_query_dsitribution/cifar10/normal_cifar10_normal_local_autozoom.png}
            \caption[]%
            {Target Model: Standard CIFAR10, Local Model: NA, NB, NC}  
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/adv_orig_query_dsitribution/cifar10/normal_cifar10_robust_local_autozoom.png}
            \caption[]%
            {Target Model: Standard CIFAR10, Local Model: R-ResN, R-DenseN}    
            
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/adv_orig_query_dsitribution/cifar10/robust_cifar10_normal_local_autozoom.png}
            \caption[]%
            {Target Model: Robust CIFAR10, Local Model: NA, NB, NC}    
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/adv_orig_query_dsitribution/cifar10/robust_cifar10_robust_local_autozoom.png}
            \caption[]%
            {Target Model: Robust CIFAR10, Local Model: R-ResN, R-DenseN}    
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/adv_orig_query_dsitribution/imagenet/autozoom.png}
            \caption[]%
            {Target Model: Standard ImageNet}    
            %
        \end{subfigure}
        \vskip\baselineskip
        \quad
        \caption[]
        {AutoZOOM Attack: Query Distribution Comparison of Starting from Local AE and Original Seed: \footnotesize{Images are sorted based on their query number of starting from the original seed}} 
        \label{fig:adv_orig_query_autozoom}
    \end{figure*}
    

\section{Seed Prioritization on Hybrid Attack}
\label{appex_sec:complete_hybrid_batch}

% \subsection{First and Second Stage of Two-Stage Strategy}
% In this section, we provide quantitative information regarding the performance of seed prioritization strategies in the first and second stage. Information of first stage prioritization metric can be found in Table \ref{appex_tab:first_stage_comp}. Information of second stage metric can be found in Section \ref{appex_tab:second_stage_comp}.

% \begin{table*}[]
% \centering
% \begingroup
% \setlength{\tabcolsep}{0.75em}
% \renewcommand{\arraystretch}{1.0}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \begin{tabular}[c]{@{}c@{}}Local\\ Models\end{tabular} & Metric & First AE & \begin{tabular}[c]{@{}c@{}}Top\\ 1\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Top\\ 2\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Top\\ 5\%\end{tabular} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}NA\\ NB\\ NC\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Transfer\\ PGD-Steps\end{tabular} & 1 & 20 & 63 & 261 \\ \cline{2-6} 
%  & \begin{tabular}[c]{@{}c@{}}Transfer\\ Random\end{tabular} & 1 & 107 & 212 & 528 \\ \cline{2-6} 
%  & \begin{tabular}[c]{@{}c@{}}Exhaustive\\ PGD-Steps\end{tabular} & 1 & 1,582 & 2,330 & 5,662 \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}R-ResN\\ R-DenseN\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Transfer\\ PGD-Steps\end{tabular} & 1 & 12 & 25 & 64 \\ \cline{2-6} 
%  & \begin{tabular}[c]{@{}c@{}}Transfer\\ Random\end{tabular} & 1 & 26 & 50 & 124 \\ \cline{2-6} 
%  & \begin{tabular}[c]{@{}c@{}}Exhaustive\\ PGD-Steps\end{tabular} & 1 & 278 & 972 & 4,555 \\ \hline
% \end{tabular}
% \caption[]%
% {Madry Robust CIFAR10 Model: Comparisons of Different Metrics in First Stage of the Two Stage Strategy}
% \label{appex_tab:first_stage_comp}
% \endgroup
% \end{table*}

% \subsection{More Results on Prioritizing Seeds in Hybrid Attack (Overall Comparison)} 
In this section, we provide a complete list of results showing the prioritization performance on hybrid attack. Details of AutoZOOM and NES attack can be found in Figure \ref{fig:batch_hybrid_nes} and Figure \ref{fig:batch_hybrid_autozoom} separately.  

    \begin{figure*}[ht]
        \centering
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/batch_hybrid/mnist/normal_mnist_nes.png}
            \caption[]%
            {Target Model: Standard MNIST\newline}    
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}
            \centering
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/batch_hybrid/mnist/robust_mnist_nes.png}
            \caption[]%
            {Target Model: Robust MNIST\newline}    
            %\label{fig:adv_orig_query_normal_cifar10}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/batch_hybrid/cifar10/normal_cifar10_normal_local_nes.png}
            \caption[]%
            {Target Model: Standard CIFAR10, Local Model: NA, NB, NC}  
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/batch_hybrid/cifar10/normal_cifar10_robust_local_nes.png}
            \caption[]%
            {Target Model: Standard CIFAR10, Local Model: R-ResN, R-DenseN}    
            
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/batch_hybrid/cifar10/robust_cifar10_normal_local_nes.png}
            \caption[]%
            {Target Model: Robust CIFAR10, Local Model: NA, NB, NC}    
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/batch_hybrid/cifar10/robust_cifar10_robust_local_nes.png}
            \caption[]%
            {Target Model: Robust CIFAR10, Local Model: R-ResN, R-DenseN}    
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/batch_hybrid/imagenet/nes.png}
            \caption[]%
            {Target Model: Standard ImageNet}    
            \label{fig:hybrid_batch_nes_imagenet}
        \end{subfigure}
        \vskip\baselineskip
        \quad
        \caption[]
        {NES Attack: Performance of Seed Prioritization on Hybrid Attack.} 
        \label{fig:batch_hybrid_nes}
    \end{figure*}
    
    \begin{figure*}[ht]
        \centering
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/batch_hybrid/mnist/normal_mnist_autozoom.png}
            \caption[]%
            {Target Model: Standard MNIST\newline}    
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}
            \centering
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/batch_hybrid/mnist/robust_mnist_autozoom.png}
            \caption[]%
            {Target Model: Robust MNIST\newline}    
            %\label{fig:adv_orig_query_normal_cifar10}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/batch_hybrid/cifar10/normal_cifar10_normal_local_autozoom.png}
            \caption[]%
            {Target Model: Standard CIFAR10, Local Model: NA, NB, NC}  
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/batch_hybrid/cifar10/normal_cifar10_robust_local_autozoom.png}
            \caption[]%
            {Target Model: Standard CIFAR10, Local Model: R-ResN, R-DenseN}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/batch_hybrid/cifar10/robust_cifar10_normal_local_autozoom.png}
            \caption[]%
            {Target Model: Robust CIFAR10, Local Model: NA, NB, NC}    
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/batch_hybrid/cifar10/robust_cifar10_robust_local_autozoom.png}
            \caption[]%
            {Target Model: Robust CIFAR10, Local Model: R-ResN, R-DenseN}    
            %
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/batch_hybrid/imagenet/autozoom.png}
            \caption[]%
            {Target Model: Standard ImageNet}
        \end{subfigure}
        \vskip\baselineskip
        \quad
        \caption[]
        {AutoZOOM Attack: Performance of Seed Prioritization on Hybrid Attack.} 
        \label{fig:batch_hybrid_autozoom}
    \end{figure*}
    
\section{Individual Test of Local Model Success Number and PGD-Steps}\label{appex_sec:compare_pgd_succ_mdel_num}
We individually test the impact of number of successfully attacked local models and the PGD steps on the identifying likely-to-transfer seeds in the first stage of the two stage strategy. 

We first note that, when there are multiple models, the number of PGD iterations is ambiguous: it may refer to the number of iterations needed to attack one of the local models successfully or may refer to attack all of the local models successfully. Because of this ambiguity, to consider the impact of PGD iterations only (to choose as one of our baselines), we count the PGD iterations that successfully attack fixed number of local models (when there are $K$ local models, we only consider iterations need to attack $k$ local models, where $k=1,2,...,K$). With this setup, we compare the ``PGD step + number of successfully attacked local models'' metric used in our paper to the baselines (i.e., clean PGD step based metrics and metric based on number of successfully attacked local models). The metric proposed in the paper is mainly used to identify directly transferable seeds by querying each seed once in the sorted order based on that metric (see Section \ref{sec:seed_prior_first_stage} for details). Therefore, we choose to compare our metric to the baselines by checking their performance in identifying direct transfers. 

We observe that PGD step based metric (including the metric adopted in the paper) is better than simply relying on number of successfully attacked local models. This is because, compared to PGD step based metrics, local model number based metric leads to more images having the same number of successfully attacked local models and we have to randomly order those images because additional information is available. In addition, we also observe that, there are no significant differences in terms of our metric and the clean PGD-step based metrics, but our metric consistently performs well in different attack scenarios. The motivations of behind our metric in the paper is 1) by grouping images with their number of successfully attacked models, we can eliminate the ambiguity of PGD iterations, and 2) by prioritizing the group of seeds that attack more local models, we expect that these seeds can have better chance to transfer to the ``unknown'' target model. 


%This section is mainly to illustrate that, PGD-Steps are more discriminative than the metric of number of successfully attacked local models. It is important to note that, when there are multiple local models, the term ``PGD-Steps'' is not well defined, as it in unclear if it is referring to the PGD-Step required to successfully attack any one of the model or all of the model. We provide more details here: the PGD-Steps used in our paper works by first grouping images based on number of successfully attacked local models and images in each group are sorted based on the PGD-Steps. The we consider the following other metrics: number of PGD steps that successfully attack $k$ of the local models, where $k$ needs to be less than or equal to the number of local models. We also compare the metric of only prioritizing based on the number of successfully attacked local models. Results are shown in Figure \ref{fig:compare_pgd_succ_mdel_num}. The overall conclusion is that, PGD-Steps are more discrminative than the number of successfully attacked local models. In addition, in terms of the metrics based on PGD-Steps, there are no significant difference among them. 

    \begin{figure*}[ht]
        \centering
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/separate_test_succ_num_pgd/mnist_normal.png}
            \caption[]%
            {Target Model: Standard MNIST\newline}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}
            \centering
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/separate_test_succ_num_pgd/mnist_robust.png}
            \caption[]%
            {Target Model: Robust MNIST\newline}    
            %\label{fig:adv_orig_query_normal_cifar10}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/separate_test_succ_num_pgd/cifar10_normal_target_normal_local.png}
            \caption[]%
            {Target Model: Standard CIFAR10, Local Model: NA, NB, NC}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/separate_test_succ_num_pgd/cifar10_normal_target_robust_local.png}
            \caption[]%
            {Target Model: Standard CIFAR10, Local Model: R-ResN, R-DenseN}    
            
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/separate_test_succ_num_pgd/cifar10_robust_target_normal_local.png}
            \caption[]%
            {Target Model: Robust CIFAR10, Local Model: NA, NB, NC}    
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/separate_test_succ_num_pgd/cifar10_robust_target_robust_local.png}
            \caption[]%
            {Target Model: Robust CIFAR10, Local Model: R-ResN, R-DenseN}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.33\textwidth}  
            \centering 
            \includegraphics[width=\textwidth,height=4.5cm]{imgs/revision_imgs/separate_test_succ_num_pgd/imagenet.png}
            \caption[]%
            {Target Model: Standard ImageNet}
        \end{subfigure}
        \vskip\baselineskip
        \quad
        \caption[]
        {Comparison of Metrics based on PGD Steps and Number of Successfully Attacked Local Models: \footnotesize{Line ``PGD+Succ-Model-Num'' denotes the seed prioritization metric used in the paper. Line ``Succ-Model-Num'' denotes the metric of prioritizing seeds only based on the number of successfully attacked local models. Line of ``PGD-Step ($i$ Local)'' denotes the prioritizing seeds based on the PGD steps taken to successfully attack $i$ number of local models. Maximum value $i$ corresponds to the number of local models}} 
        \label{fig:compare_pgd_succ_mdel_num}
    \end{figure*}z

==> 11_revision_letter.tex <==
\onecolumn

\setlength{\parindent}{0em}
\setlength{\parskip}{1em}

\section{Revisions}

This appendix describes the revisions we made to the paper \#329, entitled ``Improving Black-box Attacks on Classifiers by Combining~Transfer~and~Gradient~Attacks''. We thank all the reviewers for their constructive feedback. 

We first address the major revision criteria given in the meta-review (Section \ref{appex_sec:primary_challenge}). Then, we summarize other major improvements made in the revised version (Section \ref{appex_sec:major_change}). We provide detailed responses to the individual comments in each review in Section \ref{appex_sec:individual}. 

%\dnote{this needs to be written in a way that makes it clear that (1) here's what we understand from the reviews, (2) what we did to fix it, and (3) what the changes to the paper are.}

\subsection{Meta-review Criteria}\label{appex_sec:primary_challenge}
We address the following four criteria (Criteria 1 -- Criteria 4) given by the meta-review comments.

\subsubsection{Criteria 1: Conduct experiments to test each hypothesis/method separately, before combining multiple methods}

We propose three hypotheses in the paper and also propose an efficient batch attack method, and agree with the suggestion to evaluate each hypothesis/method separately (unlike the analysis in the original submission, which only provided a combined analysis for some of the hypotheses).

Since this criteria is based on the comments from review D, for a better linkage, we adopt the notations used in that review. We denote three hypotheses as H1, H2 and H3, and their corresponding algorithmic strategies as A1, A2 and A3. Following the notion of reviewer D, we denote the implicit Batch attack hypothesis as H4, and its algorithmic strategy as A4. (We do not consider the Batch attack an explicit hypothesis or state it this way in the paper, since several hypotheses are necessary to enable the batch attack, but agree with the reviewer that it makes sense to separate things this was so the batch attack method has a corresponding hypothesis).

In summary, the specific meaning of the hypotheses and the corresponding algorithmic strategies are (H1--H3 are stated in the paper in Section~\ref{sec:hybrid_attack}, H4/A4 is Section~\ref{sec:batch_attack}):
\begin{itemize}
    \item \textbf{H1}: local AEs are better starting points for gradient attacks. \textbf{A1}: the chosen gradient black-box attack (e.g., NES, AutoZOOM) starts from local AEs instead of the original seeds.  
    \item \textbf{H2}: label by-products generated during the gradient attack process can be used to fine-tune local models. \textbf{A2}: store the label by-products produced during gradient black-box attacks on a specific seed and fine-tune local models after the attack on that seed is done.  
    \item \textbf{H3}: gradient of local models can help with gradient based black-box attacks. \textbf{A3}: no corresponding methods, since we did not find support for this hypothesis or a useful ways to use the local gradients.
    \item \textbf{H4}: easy seeds can be identified by target model and local model information. \textbf{A4}: prioritize easy-to-attacks based on target and local model information and attack those seeds first.
    \item \textbf{Baseline}: baseline means the chosen gradient black-box attack (e.g., AutoZOOM, NES), starting from the original seed, with seeds selected in random order from the pool of seeds during the attack process. 
\end{itemize}

Among the three hypotheses, we find that H1 holds broadly, H2 only holds for smaller dataset (MNIST in our paper) and we did not find useful evidence that H3 will work. Because of this, we did not develop any method corresponding to hypothesis H3.  That said, we don't claim our failed attempts to validate and use H3 are enough to conclude that there is no way to use the local gradients, and agree with Reviewer A that it is an interesting research problem to explore this further.

Based on the notations above, we discuss the experiments on evaluating each remaining hypothesis (H1, H2, H4) and corresponding method (A1, A2, A4) independently next. 

\begin{enumerate}
    \item Impact of starting from local candidate AEs --- \textbf{Baseline} vs. \textbf{Baseline + A1}: 
    %\dnote{please don't use mysterious codes without explanation here, explain what A1 is without needing to search for it in the paper. I don't actually find it - maybe you mean H1? Either way, you need to write in a way that is easy to read and understand without assuming people will jump around trying to decode your text. I thought I made this clear in the earlier email, but I guess not.}
    
    This was actually included in the original submission, but we did not make it clear enough in the explanation. The results in Table \ref{tab:hypo_loc_adv_sample} do compare Baseline with Baseline + A1 (testing H1).\footnote{We believe the reviewer interpreted it as comparing  (Baseline + A2 + A3) and (Baseline + A1 + A2 + A3), and the text in the original submission was ambiguous so this confusion is understandable. We have rewritten the text and table caption to make it more clear.}  The prose in Section~\ref{subsec:valid_hypo} (and results in Table \ref{tab:hypo_loc_adv_sample}) compares Baseline with (Baseline + A1) --- the only difference here is whether the starting point is the original seed or a locally-generated candidate adversarial example. Specifically, we compare their attack success rate (see columns ``Baseline Success Rate'' and ``Hybrid Success Rate''), average query cost (i.e., cost per misclassified example, see columns ``Baseline Mean Query'', ``Hybrid Mean Query'') and average query cost of not directly transferable examples (see columns ``Non-Transfer Baseline Mean Query'', ``'Non-Transfer Hybrid Mean Query').  The results show the validity of H1, and impact of A1 method, across several datasets, both normal and robust models, and using different gradient-based black-box attacks.
    
    %Table \ref{tab:hypo_loc_adv_sample} compares the chosen black-box attack starting from original seeds, where seeds are selected at random , to the case of gradient attack starting from local AEs and seeds are still selected at random. Therefore, Table \ref{tab:hypo_loc_adv_sample} is a comparison of Baseline and Baseline + A1. %\dnote{again, I don't see A1, A2, A3, A4 in the paper or in Table 1}
    
    %Baseline denotes the chosen gradient black-box attack (i.e., AutoZOOM, NES) starts from the original clean image and (Baseline + A1) denotes the chosen gradient black-box attack starts from the local adversarial example. Considering A2 means that local models will be fine-tuned along the process while in Table \ref{tab:hypo_loc_adv_sample} the local model is kept static. A3 actually does not exists because we did not find useful ways to incorporate H3. A4 means easy seeds will be prioritized first by some metric, while in Table \ref{tab:hypo_loc_adv_sample}, seeds are selected at random. 
    %Then, in Table \ref{tab:hypo_loc_adv_sample}, we measure their performance in terms of attack success rate, mean number of query cost and fraction worse (i.e., seeds can be attacked more efficiently by starting from the original seed instead of the local AE). We add more clarification in the caption of Table \ref{tab:hypo_loc_adv_sample} to avoid confusion.
    %\dnote{I can't make any sense of what is written here. Please focus on responding to the reviewer comment - this should be either explaining why it isn't reasonable to do what they asked, or how you tested each hypothesis separately, and summarizing the method and results here, and pointing to where in the paper they are now presented.}
    
    
    \item Compare Baseline to Baseline attack with local models fine-tuned by its label by-products --- \textbf{Baseline} vs \textbf{Baseline + A2}: 
    
    The original submission consider the impact of A2, but didn't separate this from A1 (that is, the experiments testing the local model tuning all assuming the attack would start from a local candidate AE). Following the reviewers suggestion, we conducted new experiments to test this hypothesis independently. We provide experimental results for the comparison of Baseline and (Baseline + A2) in Table \ref{tab:hypo_2_validate} and discuss in Section~\ref{sec:loc_model_tune}. Specifically, we rerun the gradient attack starting from original seeds, store the label by-products during the process and fine-tune the local models periodically. We report the transfer rate of the local models before and after the fine-tuning process. We only report the transfer rate of local models because, the gradient attack in (Baseline + A2) starts from the original seed and therefore is identical to Baseline attack in terms of query cost and attack success rate. The results are consistent with the results we had found previously when testing in combination with A1: A2 still helps for MNIST (i.e., increases the transfer rate of tuned local models) but fails on CIFAR10 (the transfer rate of tuned local models actually decreases). This is consistent with what we showed in Section 4.5 in the original submission where we compared the case of hybrid attack with static local model (i.e., Baseline + A1) to the case of hybrid attack with fine-tuned local model (i.e., Baseline + A1 + A2). A1 (gradient attack starts from local AEs) is considered in both sides of comparison because, we need to start from local AEs such that, when local models are fine-tuned, we can potentially benefit from the better local AEs generated from the fine-tuned local models. As shown in Table \ref{tab:hypo_fine_tune}, the results for the isolated A2 experiment are similar, showing that A2 works for MNIST but fails on CIFAR10. 
    

    \item Compare Baseline to Baseline attack where images are prioritized based on target loss value --- \textbf{Baseline} vs \textbf{Baseline + A4}: 
    
    The experiments in the original submission showed the impact of the batch attack (A4), but in combination with the other methods. We have added new experiments that consider the batch attack separately when possible, assuming that the only aspects used from other methods are how seeds are prioritized and not how the attack is done. (In some cases, separating the prioritization from the attack method doesn't make sense, since the prioritization based on the local candidate AEs only makes sense if the attack also uses the local candidate AEs.)
    
    In the case of (Baseline + A4), the attacker can prioritize easy seeds based on the target loss function value. Note that, PGD steps or other local model information cannot be used here for seed prioritization because this baseline does not use any local models. We rerun the experiments and present the comparison of Baseline and (Baseline + A4) for AutoZOOM attacks on the Madry robust CIFAR10 model and standard ImageNet model in Section \ref{sec:prior_metric_eval} (Figure \ref{fig:h4_test_autozoom_main_cifar10} and Figure \ref{fig:h4_test_autozoom_main_imagenet}). These two target models are selected to represent the cases where prioritization succeeds and fails. A complete list of results are shown in in Figure \ref{fig:h4_test_nes} (based on NES attack) and Figure \ref{fig:h4_test_autozoom} (based on AutoZOOM attack) in Section \ref{appex_sec:h4_baseline} of the Appendix. The results are mostly similar to the batch attack results for the hybrid attack that, prioritizing based on target function value has closer performance to the retroactive optimal strategy and is much better than randomly scheduling the seeds. One exception happens for AutoZOOM attack on ImageNet target model, where H4 + baseline does not improve significantly compared to random scheduling of the baseline (see Figure \ref{fig:h4_test_autozoom_main_imagenet}). However, their corresponding ImageNet part of hybrid attack (i.e., Baseline + A1 + A4) has much better prioritization performance compared to random scheduling (see Figure \ref{fig:hybrid_batch_autozoom_main_imagenet}). We believe this interesting phenomenon happens because, for natural images, the models tend to ``overfit'' and therefore, target loss computed for that seed becomes less expressive in terms of representing the attack difficulty. In constrast, local AEs are perturbed from the natural images, and therefore, models are less likely to overfit to perturbed images. Because of this, target loss values are more representative of their true attack difficulty. Detailed discussion and explanation about this phenomenon is presented at the end of Section \ref{sec:prior_metric_eval}.   
\end{enumerate}

\subsubsection{{Criteria 2: Report both the number of queries and success rate, in addition to the average query cost per misclassified example.}}

This criteria is based on the comment from review D: \textit{I would have liked to see you report the raw numbers of number of model queries and number of successes, instead of reporting only the ratio. Has the cost computation been applied consistently to everything, including the baseline? To compare fairly, you'll need to multiply the number of queries for the baseline by its success rate (if the baseline takes 1000 queries on average and succeeds 50\% of the time, then you need to use a cost of 500 as the comparison point, not 1000). I can't tell whether that has been done, and I dont' see the cost of the baseline reported.}


We have added the (raw) ``number of queries'' in Table \ref{tab:hypo_loc_adv_sample} and Table \ref{tab:hypo_fine_tune} following the suggestion of reviewer D. We also replace the ``Mean Reduction in Queries'' with actual mean query of hybrid attack in Table \ref{tab:hypo_loc_adv_sample}. The cost of baseline is reported in Table \ref{tab:hypo_loc_adv_sample} (see column ``Baseline Mean Query''). 

To clarify, all the attack success rates are reported in all of our results using the same cost computation criteria (i.e., average cost per successful adversarial example found). This is applied consistently for both the baseline and hybrid strategies (see columns of ``Baseline Success Rate'' and ``Hybrid Success Rate'' in Table \ref{tab:hypo_loc_adv_sample} and columns of ``Success rate for static local model'' and ``Success rate for tuned local model'' in Table \ref{tab:hypo_fine_tune}).  

Although previous work in this area has typically excluded failed attempts in their cost reporting (that is, previous works often report average number of queries used for searches for seeds that eventually result in successful adversarial examples), we think this metric is less useful and potentially misleading. The adversary doesn't know if a candidate seed will eventually lead to a successful adversarial example, so all the queries made to the target model should count---excluding queries for seeds that don't eventually lead to a successful adversarial example distorts the results and misrepresents the actual attack cost. 

To use the example in the review comment, if the baseline takes 1000 queries on average when it succeeds, and succeeds 50\% of the time, the actual cost of the attack per successful adversarial example would be $(1000 + T)/2$ where $T$ is the (fairly arbitrary) maximum number of queries threshold before giving up. Reporting the cost using just the average number of queries used for the successful attempts means attacks with lower average number of queries and lower attack success rate will lead to lower final cost, which contradicts the attacker's goal in finding efficient attacks with lower number of queries and higher success rate (in the extreme, it would result in an attack cost of 1, where only successful direct transfers are considered, and no gradient searching is done). In contrast, we consider the primary metric to be ``average query cost per successful adversarial example found'' (which is simply computed as the total number of queries divided by the total number of adversarial examples found.  This metric gives lower cost to attacks with lower number of queries and higher success rates. Because of this, we believe this metric aligns well with the attacker's goal and we focus on this metric in most of our discussions in the paper. 

\subsubsection{{Criteria 3: Explain how the local models are trained and how the byproducts of the black-box attack are used to train the local models.}}

We have added details on how the by-products of gradient black-box attack are used to fine-tune the pretrained local models during the attack process at the end of Section \ref{sec:hybrid_attack}. In addition, we also update Algorithm \ref{alg:hybrid} to provide more details on the tuning (line \ref{line:tuneset} and line \ref{line:auugmenttuneset}).

In terms of the initial local model (before the attack starts), we adopt standard CNN models, which are individually trained on standard MNIST, CIFAR10 and ImageNet training data. We believe the confusion about our local models resulted from the unclear definition of the threat model in the original submission, so we have clarified our threat model at the beginning of Section \ref{sec:hybrid_attack}.

\subsubsection{{Criteria 4: Address the other specific comments in the reviews on writing and presentation, where possible.}}
We have updated the paper content based on reviewer comments.  Section \ref{appex_sec:individual} provides detailed responses explaining how we revised the paper in response to each specific reviewer comment. We also made some other improvements and changes to the overall presentation to improve clarity, which we describe in Section~\ref{appex_sec:major_change}.

\subsection{Other Major Changes}\label{appex_sec:major_change}

\subsubsection{Improving Effectiveness against Robust CIFAR10 Models}

Both review A and reviewer B pointed out the ineffectiveness of our attacks against the robust CIFAR10 models. We agree that it is essential to understand attacks when the target model is designed to be robust, since presumably that will (eventually) be the scenario that is more relevant. 

Our work over the past few months has focused on understanding this, and we have found ways to improve the attack against robust models. The main issue is that robust models seem to have different attack surfaces from non-robust models, so the local candidate AEs generated from local non-robust models did not provide useful starting points. To tackle the ineffectiveness of hybrid attack against the robust CIFAR10 model, we adversarially train two deep CIFAR10 models and redo the experiments with robust local models (see Section \ref{sec:improve_robust_attack}). All results support our claim that different attack surfaces of robust and local models seem to be the main reason and we can improve effectiveness against robust CIFAR10 target model by adopting robust local models.

\subsubsection{Presentation of Batch Attack Strategy}

We realize from the reviews that the way we presented the batch attack was confusing (Section 5 in the original submission and revised version), and have rethought how to present this to improve clarity and simplify the attack description. Now, we frame the batch attack strategy as a two-stage strategy, where in the first stage, local model information is utilized to find likely-to-transfer seeds and target model information is utilized to find easy-to-attack seeds in the second stage. Although this seems to restrict the attack from the most general case where each query could be used to either attempt a local transfer on a new candidate or to follow a gradient attack strategy, in our experiments the expected cost of a potential transfer is so much lower than a gradient attack that we concluded the extra generality is not worth the complication of combining the attacks, and it is simpler to just view the attack as having two phases: first try to find successful direct transfers, and then do gradient-based attacks starting from the candidates.  This change does not impact the batch attack results, but allows for a simple presentation of both the attack and experimental results.

In order to have better flow in discussing the two-stage strategies and their evaluations, Section 5 and Section 6 in the original submission are merged to a single Section \ref{sec:batch_attack}. We also delete the comparison of hybrid strategy and baseline strategy in the batch attack setting (Section 6.2 in original submission). The reason is that the hybrid strategy already outperforms baseline attacks significantly (in terms of attack success rate, average query cost as shown in Table \ref{tab:hypo_loc_adv_sample}), and therefore, it is unnecessary to illustrate its effectiveness in batch attack setting again. 

\subsubsection{Restricted Black-Box Settings}

Reviews A and C suggested considering attack settings there the query result provides limited information, such as only the top-k class confidence scores or only the output label. We agree that it would be interesting to explore applicability of our attack strategy in more restricted black-box settings, but leave this for future work. We are optimistic that our methods will provide benefits for these restricted attacks because the hybrid attack boosts existing attacks by providing better starting points for the attacks (e.g., generated local AEs) and from our experiments, we have shown that it is effective for several different attacks. We also emphasized in the paper that having full prediction vector is a stronger assumption compared to partial observations or label only observations (see the end of Section \ref{sec:other_grad_attacks}). 

\subsubsection{Results of NES-Bandits Attack}
In the original submission, we did not include results of the NES-Bandits attack (an improved version of the NES attack) \cite{ilyas2018prior}. In the revised version, we have added results of the NES-Bandit attack on ImageNet in Table \ref{tab:hypo_loc_adv_sample}. (The source code of NES-Bandit attack only contains evaluation on ImageNet, so we have not included results for MNIST or CIFAR10.) For NES-Bandits, the improvement of the hybrid attack (i.e., starting from the local AEs) is significant over the baseline attack (i.e., starting from the original seed), and the mean cost reduction is over 80\% (see Table \ref{tab:hypo_loc_adv_sample}). This is a significant improvement, but we also observe that NES-Bandits is not performing as well as NES or AutoZOOM attack in targeted attacks on ImageNet model (the original paper only evaluates untargeted attacks on VGG ImageNet model, and demonstrated that NES-Bandits outperform NES significantly on that model). Since our goal in this work is to show the impact of the hybrid attack strategy on the different black-box gradient attacks, we did not investigate this further (for this paper), but plan to do more experiments to understand the variation between these attacks on different models in future work.

%\snote{I guess we do not need this...} In our experiments, we conduct targeted attacks (with least likely class as the target class) on DenseNet ImageNet model and therefore, we are unable to do a sanity check in terms of performance of the Baseline NES-Bandit attack. For a more fair comparison, we are in the process of implementing our hybrid attack framework in the exact same setting of \cite{ilyas2018prior} and will include more results in the future version.  


\subsection{Individual Responses}\label{appex_sec:individual}
In this section, we respond to comment from each reviewer point by point. To avoid repetition, we removed some comments that are addressed in previous section. 

\subsubsection{Review A}
\shortsection{Comment 1: \rm\it My main concern is the presentation of results and how the query-efficiency comparison is made with prior black-box attacks. In particular, the hybrid approach presented here makes the assumption that an ensemble F of local models is available to the adversary (see Algorithm 1). This assumption is equivalent to the setup cost of transferability-based attacks: this model extraction would make up all of the query cost of transferability-based attacks. Hence, the current manuscript should explicitly state that assuming availability of this local ensemble should be taken into account as part of the query budget spent by the adversary to mount the hybrid attack presented here. Note however that the increased cost is acceptable, because the quality of the hybrid attack is higher compared to a vanilla transferability-based attack. Thus, if this paper were to be accepted, a better way to frame the results would be that the success rate of a transferability-based attack can be enhanced using finite-difference queries to compute better approximations of gradients once a good candidate seed has been identified on the local model%This assumption is equivalent to the setup cost of transferability-based attacks: this model extraction would make up all of the query cost of transferability-based attacks. Hence, the current manuscript should explicitly state that assuming availability of this local ensemble should be taken into account as part of the query budget spent by the adversary to mount the hybrid attack presented here. Note however that the increased cost is acceptable, because the quality of the hybrid attack is higher compared to a vanilla transferability-based attack. Thus, if this paper were to be accepted, a better way to frame the results would be that the success rate of a transferability-based attack can be enhanced using finite-difference queries to compute better approximations of gradients once a good candidate seed has been identified on the local model. 
} 
%For instance, on MNIST and CIFAR10, would the query budget for the hybrid batch attack exceed (or be in the order of) the number of labels needed to train a substitute model?}

Reviewer A suggests to consider the setup cost of extracting the local model into the query cost computation of hybrid attack, and then compare to other attacks. 

Setup cost is an important factor to consider when the attacker needs access to local models. For this work, we have assumed the attacker has access to pretrained local models (this is the same assumption as most previous work on transfer-based attacks), which indicates that attacker knows both the training data and local model architecture, and the setup cost here refers to the computational resources spent to train the local models. We have clarified our threat model to make this clear (at the beginning of Section~\ref{sec:hybrid_attack}) and added a discussion about the setup cost (at the beginning of Section~\ref{sec:hybrid_evaluation}).  

We agree with the reviewer that in many scenarios it is not realistic to assume the attacker has ready access to pretrained local models, and it would be valuable to incorporate the cost of producing such models in the attack cost model. The actual cost of this, however, is very hard to estimate and highly application and attacker specific --- it depends on the costs of acquiring training data, how much effort would be required to find a good model architecture and determine hyperparameters, and the compute resources available to the attacker. Further, the setup cost is a one-time cost, which becomes dominated by per example cost when large number of seeds are attacked. Hence, we only consider per-example attack cost when comparing to baseline gradient attacks. 

Following the reviewer's suggestion, in Section \ref{subsec:valid_hypo}, we also highlight that our hybrid attack strategy boosts transfer based attacks by better estimating the target model gradients with fine-difference methods, and starting from non-transferable but still good seeds.

\shortsection{Comment 2: \rm\it Related to this, it would be useful for the presentation to put the number of queries performed by the hybrid approach in context with the size of the training set needed to learn the substitute (extracted) model in a vanilla transferability-based attack. For instance, on MNIST and CIFAR10, would the query budget for the hybrid batch attack exceed (or be in the order of) the number of labels needed to train a substitute model?}

This confusion still results from the unclear definition of threat model in the original submission, and the difficulty in estimating setup cost in cases where the adversary does not have access to pretrained models. We clarify that, in our threat model, we assume the training data is available to the attacker so attackers can train reasonable local models without needing any query interaction with the target model. Therefore, the setup cost, which is the computational resources to train local models, is not comparable to the per-example cost. 
It is also helpful to note that our assumption on local models (which is the same assumption used in most transfer attacks) is different from the weaker assumption made in the substitute training approach \cite{papernot2017practical}, which only assumes having access to randomly initialized local models and a small amount of training data which is then augmented by interacting with the target model (model extraction problem). The problem with substitute training approach is, there is currently no clear evidence that it can work for complex datasets (even for CIFAR10 such attacks have not been very successful). In our hybrid attack framework, we also tried the weaker assumption of only having access to randomly initialized local models, but failed to make it work for CIFAR10 dataset (it only succeeds on MNIST, which does not provide confidence that it could work in general).

\shortsection{Comment 3: \rm\it Expanding on this particular limitation, the average query cost per misclassified example might not be the right metric given that transferability attacks have a large upfront cost but a low per example cost, whereas finite-difference gradient based attacks are the opposite: they have zero upfront cost but a large per example cost. Computing the mean query cost also prevents us from separating individual factors like success rate and per example number of queries: for instance in Table 1, it is hard to tell which part of the mean query reduction is due to the attack being more successful and which part is due to the finite-difference gradient-based attack being bootstrapped with an adversarial examples computed on the local ensemble F. Visualizing the query distribution like Figure 2 does for other results in the paper would help provide more insights to the reader} 
%like success rate and per example number of queries: for instance in Table 1, it is hard to tell which part of the mean query reduction is due to the attack being more successful and which part is due to the finite-difference gradient-based attack being bootstrapped with an adversarial examples computed on the local ensemble F. Visualizing the query distribution like Figure 2 does for other results in the paper would help provide more insights to the reader.}

%\dnote{I think this is a convoluted response, where there should be a simple one that says how the paper was improved based on this comment.}
To distinguish the impact of direct transfers and the benefits of gradient-based attack being boosted with local AEs, we added mean query cost of the non-direct transfers (See Columns ``Non-Transfer Baseline Mean Query'' and ``Non-Transfer Hybrid Mean Query'' in Table \ref{tab:hypo_loc_adv_sample}). In addition, we plot the query distribution of starting from original seed and local AE in Figure \ref{fig:adv_orig_query_nes} (for NES attack) and Figure \ref{fig:adv_orig_query_autozoom} (for AutoZOOM attack). 

%We note that images in each figure are sorted based on the query number of the attack that starts from the original seeds. More Quantitative information regarding Figure Figure \ref{fig:adv_orig_query_nes} and Figure \ref{fig:adv_orig_query_autozoom} can be referred to Table \ref{tab:hypo_loc_adv_sample}.
%Reviewer A suggests to distinguish the saved query cost resulted from directly transferable samples and the non-direct transfers that boost gradient attacks. Reviewer A Also suggests to visualize the query distributions of attacks starting from a given image and starting from the local AE of that image.  
%Since the setup cost is not considered as a main cost, we believe the average query cost per misclassified example is still a reliable metric to evaluate different attacks. To distinguish between  in Table \ref{tab:hypo_loc_adv_sample}, we . 

\subsubsection{Review B}
\shortsection{Comment 1: \rm\it The authors try to combine transfer and gradient-based black-box attacks to improve black-box attacks. However, the contribution is incremental and the combined attack has limited effectiveness for defended models}

Since the original submission, we have improved the effectiveness of our attack against the robust CIFAR10 model by adopting adversarially trained robust local models and added a new section on this to the paper (Section \ref{sec:improve_robust_attack}). For example, when attacking robust CIFAR10 model with AutoZOOM attack, in the original submission, the mean cost reduction compared to the baseline attack is only 4.1\%, but with robust local models, the mean cost reduction can be improved to 21\%. We also observe significant decrease in the fraction worse (from 25.6\% of normal local models to 4.4\% of robust local models). Attack success rate of the gradient attack is also improved slightly (from 65.2\% of normal local models to 68.7\% of robust local models and the baseline success rate is only 64.4\%).

%Our contribution is the first work to combine transfer and gradient attacks, which although it may seem incremental, has not been considered by previous researchers, and the research has bifurcated into the two types of attacks that are strangely treated as independent from each other. Our hybrid attack also improves state-of-the-art results significantly on standard deep learning models and we demonstrate that real-world attackers can be much more destructive than expected. We also consider a more practical query limited batch attack setting and propose efficient and effective seed prioritization methods to further improve query efficiency of gradient black-box attacks.   

\shortsection{Comment 2: \rm\it
Details about the tuning part is missing. How are the byproducts of black box attack used to retrain local models? Are they used as the only training data when tuning, or are they added to the original training set and mix up, or are they added to each batch?}

We have added details on the local mode fine-tuning in Section~\ref{sec:loc_model_tune}.

\subsubsection{Review C}
\shortsection{Comment 1: \rm\it I was confused about the term "original seed". Do you mean randomly initialized seed? Or something else? Also, In algorithm 1, does "Candidate seeds" again refer to random initializations or something else?}

In the paper, we assume attacker starts with a pool of seed images. This is the same assumption made in most adversarial machine learning research. ``Original seed'' means an image in the initial pool of seed images, which are natural examples correctly classified by the target model. 

In the original submission, we made a confusing statement about ``Candidate seeds $\mathbf{X}$'' when describing Algorithm \ref{alg:hybrid}, but it actually denotes the set of natural seed images that are correctly classified by the target model. We have updated Section \ref{sec:hybrid_attack} to avoid this confusion and also changed``Candidate set $\mathbf{X}$'' to ``Set of seed images $\mathbf{X}$'' in Algorithm \ref{alg:hybrid}.  

%More generally, we name ``Candidate'' as an input image that is considered for an attempted attack on the target model. Therefore, for attack described in Algorithm \ref{alg:hybrid}, the candidate seed is the local adversarial example because we attack the target model by starting from the local AE. If the attack is the baseline attack that starts from the original seed, then candidate seed denotes the original seed instead.

%“Candidate set” in Alg 1 refers to the set of clean images. To avoid confusion, we made our statement clearer and also changed “Candidate set” to “Set of natural images” in Algorithm 1.
%\dnote{confusing answer - don't we assume the attacker starts with a pool of seed images, which are natural examples. This is the same assumption in most adversarial examples research. By "original seed" we mean an image in the initial pool of seed images which are correctly classified by the model. I think it is confusing to use "candidate" here, since we use "candidate" for the adversarial examples found against the local models - candidate should mean any input image that is considered for an attempted attack on the target model, which could mean an original seed or generated local AE}

\shortsection{Comment 2: \rm\it to algorithm 1, the text mentions that the "adversarial search space is defined in terms of the original seed x, not the starting point found using local models x`". Please clarify why this is the case, and how it impacts the algorithm. It was not immediately clear}

We added a clarification on this issue (at the end of Hypothesis 1 in Section~\ref{sec:hybrid_attack}). Specifically, constraining the space of valid adversarial examples to be the search space of original seed $x$ (i.e., the natural image) ensures that the AE found by our method still look visually similar to natural image $x$ (or, at least, that it satisfies the standard definition of an adversarial example for seed $x$). Such a constraint is important because if the search space is constrained with respect to the local AE (already a perturbed image compared to its natural image), the final AE obtained may no longer look visually indistinguishable from the natural image.  (At worst, it could be $2\epsilon$ distance from the original seed $x$, since the local AE is within $\epsilon$, and defining the search space around this local AE could include points up to $2\epsilon$ away from $x$, which would potentially double the strength of the adversary.

\shortsection{Comment 3: \rm\it In Table 1, the ImageNet gains are not as pronounced. Given that ImageNet is really the thing everyone cares about, I'm not sure whether a 23.2\% reduction in mean queries is significant. Furthermore, if there is a robustly trained ImageNet model, I would imagine that this number drops much lower (based on the trends I'm seeing in MNIST and CIFAR). Are there ways to improve this reduction in queries?}

Less reduction in queries is observed for NES attack on ImageNet because the direct transfer rate of local ImageNet models are lower (only 4.2\% while MNIST and CIFAR10 standard models have over 60\% transfer rate), which may also degrade the quality of non-transferable local AEs which can help boost the gradient attacks. Finding more transferable local models or better attacks on local models (e.g., recent works in \cite{xie2018improving,dong2018boosting,dong2019evading}) may improve the results. We also note that, in the newly added results of NES-Bandit on ImageNet (claimed as an improved version of NES in \cite{ilyas2018prior}), the query cost reduction is over 80\%. There are some attempts to build robust ImageNet models by adversarial training \cite{kannan2018adversarial} and we have not exhaustively considered all these models yet. However, their robustness is less effective compared to the ones in smaller datasets (e.g., MNIST, CIFAR10). To make our attack more effective against robust ImageNet models, we can also adopt adversarially trained local models and more discussion on this issue can be found in Section \ref{sec:improve_robust_attack}. 

% Our current “mean cost reduction” causes some confusion because it mixes the contribution of two factors: 1) direct transfers of some examples can save query efficiency, 2), non-transferable examples provide better starting points and save query efficiency.
% To distinguish their individual effect, we added two more columns in Table 1 to measure the query efficiency of non-transfers. 

\shortsection{Comment 3: \rm\it in Table 2, there appears to be a confusing result. For CIFAR 10, it appears that the mean query cost for the tuned local model increases compared to the cost for the static local model. This is quite confusing -- does it imply that the attack has somehow become more difficult? Please clarify this discrepancy in future versions of the paper}

Yes! It is indeed the case that fine-tuning the local model appears to actually worsens the attack quality. This observation leads to our conclusion that fine-tuning local models currently does not work well for larger dataset (e.g., CIFAR10) (that is, Hypothesis 2 does not hold). We have updated the discussion of this issue at the end of Section \ref{sec:loc_model_tune} with a more explicit statement. We also tried several other tricks to circumvent this issue (e.g., only fine-tuning the local model based on newly generated label by-products), but nothing we tried worked. We suspect that the failure stems from the complexity of the dataset itself and leave further explotation for future work.

\subsubsection{Review D}
\shortsection{Comment 1: \rm\it I would have liked to see a clearer description of
the experimental methodology. What attacks did you
implement, and how were they conducted? I'm confused
why NES or AutoZOOM are listed as transfer attacks in
Section 4.4}
%as Section 4.2 correctly explains, they
%are gradient attacks, not transfer attacks.}

In Table \ref{tab:hypo_loc_adv_sample}, we report direct transfer rates of local AEs, which are independent of the chosen black-box attack (i.e., NES, AutoZOOM) but later used as starting points for these gradient attacks. We reorganized Table 1 to avoid this confusion. We also added details on each of the gradient attack methods (see ``Attack Distance Metric and Magnitude'' in Section~\ref{subsec:setupattacks}).  

\shortsection{Comment 2: \rm\it The way that Algorithm 1 combines batching and H3
doesn't make sense to me.  I would not expect that
byproduts from attacks on $x_1$ would be useful for
attacks on $x_2$.  We're trying to build a local model
and the essence of that model is that it is a substitute
for the actual model that behaves similarly in the
local neighborhood of a single point.  They're local
models, not global models.  So, the labels from
attacking $x_1$ might well improve a local model to
be more accurate in the neighborhood of $x_1$, which
might be useful for attacking $x_1$; but I would not
expect them to be useful for improving accuracy in
the neighborhood of some totally other example
$x_2$}

This comment reflects some confusion, and we have tried to improve the presentation to make things clearer. We first clarify that Algorithm \ref{alg:hybrid} does not include H3, as we did not find any evidence that H3 can directly work. To incorporate batching into Algorithm \ref{alg:hybrid}, we also did not consider fine-tuning local model (alternatively, we can view it as deleting line \ref{line:tunemodels} from Algorithm \ref{alg:hybrid}) because we find that local model fine-tuning does not work well for CIFAR10 dataset (shown in section \ref{sec:loc_model_tune}) and we also do not have fine-tuning results for ImageNet. Therefore, the local models remain static during batch attacks. 

Batching is incorporated to Algorithm \ref{alg:hybrid} by replacing the \textit{selectSeed()} function (line \ref{line:selectseed} in Algorithm \ref{alg:hybrid}) with \textit{EstimateAttackCost()} in Section \ref{sec:batch_attack} such that the most promising seeds are prioritized. In addition, since the local models are static, attacks on different images are actually independent. 

\shortsection{Comment 3: \rm\it Averaging the transfer rate between AutoZOOM and
NES doesn't make sense.  Don't do that.  Report them
separately.  If you need to pick a single number,
then choose the better of the two.  An attacker isn't
going to flip a coin and choose randomly between
those two; instead, an attacker will choose the better
of them}

Local AEs are actually independent from the gradient black-box attacks --- the gradient attack only starts after the first query fails to transfer. So, the transfer rates should be exactly the same same for all the gradient attacks since they only depend on how the first candidate query is selected, this is why we don't split the transfer rates by the different gradient attack method in Table~\ref{tab:hypo_loc_adv_sample} and Table~\ref{tab:hypo_fine_tune}.  All the experiments use the same set of local AEs for each of the NES, AutoZOOM and NES-Bandit attacks in the revised version.

\shortsection{Comment 4: \rm\it I couldn't understand the meaning of some of the
columns of Table 1.  The caption doesn't appear to match the column labels}

The mismatch in Table~\ref{tab:hypo_loc_adv_sample} caption is fixed. ``Mean Reduction in Queries'' in Table \ref{tab:hypo_loc_adv_sample} is calculated as (mean query cost of baseline attack - mean query cost of hybrid attack)/(mean query cost of baseline attack). We have added more complete descriptions of each column to the caption of Table~\ref{tab:hypo_loc_adv_sample}.

\shortsection{Comment 5: \rm\it Section 4.5 reports that fine-tuning local models
improves transfer rates; I wish it had reported how
many queries were needed to achieve these improvements}

We provide the total number of input-label pairs produced during the gradient attacks, which are then used to fine-tune the local models, in Table \ref{appex_tab:label_prod_size_2}. (Because of space limits, this has been moved to the appendix.) However, it is important to note that fine-tuning local models does not need additional queries, and the input-label pairs are actually free by-product of conducting the gradient attacks. In addition, only fine-tuning MNIST local models increases the model transfer rate and fine-tuning CIFAR10 models actually decreases the transfer rate (as discussed for Review C, Comment 3). 

\shortsection{Comment 6: \rm\it Section 4.3: where you write "we choose least likely class", can you be more precise what you mean by that?}

We made our statement in Section \ref{subsec:setupattacks} more explicit in terms of the definition of least likely class. Specifically, for CIFAR10 and MNIST, since we sample 100 images from each of the 10 classes, ``least likely class" refers to the least likely class of a particular class, not a particular image. Least likely class of a given class is obtained by first getting the least likely class (i.e., the class with lowest probability predicted by the target model) of each seed in that class, and then taking the mode. For ImageNet, we randomly select 100 images (not restricted to specific classes) and the least likely class for an image is chosen as the class with lowest probability for that image. 

\shortsection{Comment 7: Section 5.2: \rm\it I wish you had separated out the benefit of prioritizing based on number of successfully attacked local attacks vs sorting by PGD iterations. How much benefit do we get from using just one or the other of those, without using them both?}

%For the convenience of presentation, we denote the metric of prioritizing based on number of successfully attacked local models as ``Succ-Model-Num''. And we name the PGD-Step based metric mention in the original submission as ``PGD + Succ-Model-Num''. 
We run experiments to check the individual impact of number of successfully attacked local models and the PGD iterations. Results are shown in Figure \ref{fig:compare_pgd_succ_mdel_num} in Section \ref{appex_sec:compare_pgd_succ_mdel_num} of the appendix (moved to appendix due to space limitation). We add discussion about this issue in Section \ref{sec:seed_prior_first_stage}. We need to make few more clarifications below such that reviewer can better interpret the results.

We first note that, when there are multiple models, the number of PGD iterations is ambiguous: it may refer to the number of iterations needed to attack one of the local models successfully or may refer to attack all of the local models successfully. Because of this ambiguity, to consider the impact of PGD iterations only (to choose as one of our baselines), we count the PGD iterations that successfully attack fixed number of local models (when there are $K$ local models, we only consider iterations need to attack $k$ local models, where $k=1,2,...,K$). With this setup, we compare the ``PGD step + number of successfully attacked local models'' metric used in our paper to the baselines (i.e., clean PGD step based metrics and metric based on number of successfully attacked local models). The metric proposed in the paper is mainly used to identify directly transferable seeds by querying each seed once in the sorted order based on that metric (see Section \ref{sec:seed_prior_first_stage} for details). Therefore, we choose to compare our metric to the baselines by checking their performance in identifying direct transfers. 

The results are unsurprising that PGD step based metric (including the metric adopted in the paper) is better than simply relying on number of successfully attacked local models. This is because, compared to PGD step based metrics, local model number based metric leads to more images having the same number of successfully attacked local models and we have to randomly order those images because no additional information is available. In addition, we also observe that, there are no significant differences in terms of our metric and the clean PGD-step based metrics, but our metric consistently performs well in different attack scenarios. The motivations of behind our metric in the paper is 1) by grouping images with their number of successfully attacked models, we can eliminate the ambiguity of PGD iterations, and 2) by prioritizing the group of seeds that attack more local models, we expect that these seeds can have better chance to transfer to the ``unknown'' target model. 


%\snote{I will revise this part again} We run separate experiments on grouping by number of successfully attacked local models and number of PGD iterations. The results are unsurprising that PGD iteration itself is better than successfully attacked local models and their combination gives the best result. Due to space limit, we provide a sample demonstration in Figure \ref{} in the appendix. 

%The results are unsurprising because the prioritization quality of identifying easy-to-attack seeds depends on how discriminative the chosen metric is. PGD is better than local model number because number of successfully local models is fairly limited (e.g., up to only 3 local models in our experiment setting) while the PGD steps can be integers up to 100 and therefore is not discriminative enough (i.e., there will be lots of images with same number of successfully attacked local models and these images can only be randomly ordered if not additional information is available). 
%Their combination gives best performance because: grouping seeds first by their number of successfully attacked local models and prioritizing seeds that attack more local models can guarantee that the perturbation does not overfit to specific models too much and can better transfer to the target model. Prioritizing seeds in each group (i.e., seeds attack same number of local models) by their PGD-Steps is more discriminative than just randomly ordering the seeds. Intuition behind these metrics are presented at the end of Section \ref{sec:seed_prior_first_stage}.




==> XX_07_batch_attack_evaluation.tex <==
%\section{Evaluation of Batch Attacks}\label{sec:batchevaluation}

    


    


%\shortsection{Demonstrating Effectiveness of Hybrid Attack in Batch Setting}
%To show the effectiveness of the hybrid attack strategy in query limited setting, we compare the hybrid attack strategy with seed prioritization to the gradient based attacks start from original seed. %and with adoption of the same seed prioritization strategy.  

% \paragraph{Retroactive optimal strategy with baseline attack} 
% For this approach, the attacker is assumed to have prior knowledge on the true rank of seeds based on their actual number of queries needed. However, when attacking each seed image with the given selected baseline method, the starting points are the original seeds.
% \paragraph{Greedy strategy with baseline attack}
% For this approach. the attacker is capable of prioritizing the seeds based on the defined loss function, but individual seed is attacked from the original seed with the given baseline attack. 

% \paragraph{Random scheduling with baseline attack} 
% For this approach, the attacker is capable ranks the seed in random order and attack on each individual seed starts from the original seed. This approach also denotes the direct application of current state-of-the-art black-box attacks in query limited setting, where attack success rate is the major metric and internal difference of different seeds are often ignored.

%We first show the impact of different seed prioritization strategy on the first-stage of the two-stage strategy (Section \ref{sec:candi_sel_eval}). Then, we demonstrate effectiveness of the complete two-stage strategy when combined with seed prioritization strategies (Section \ref{subsec:opt_two_stage}). Finally, we evaluate the performance of seed prioritized two-stage strategy in comparison to two degenerate cases (Section \ref{sec:prior_metric_eval}). 
% \begin{table*}[tbh]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% Attack Method & Prioritization Method & First AE & 1\% & 2\% & 5\% & 10\% \\ \hline
% \multirow{5}{*}{AutoZOOM} & Retroactive Optimal & 1 & 10 & 20 & 50 & 149  \\ \cline{2-7} 
%  & Attack Loss + PGD Step & 3 & 28 & 51 & 243 & 1,114  \\ \cline{2-7} 
%  & Attack Loss & 6 & 100 & 206 & 522 & 1,114 \\ \cline{2-7} 
%  & PGD Step & 530 & 1,516 & 6,272 & 8,506 & 34,332 \\ \cline{2-7} 
%  & Random & 121 & 20,647 & 43,928 & 125,147 & 246,889 \\ \hline
% \end{tabular}
% \caption{Comparison of Different Scheduling Strategies: \footnotesize{column ``First AE" denotes the query number needed to find the first adversarial example. Subsequent columns of ``x\%" denotes number of queries needed to find x\% fraction of adversarial examples out of the total candidate seeds. For ``Random" scheduling strategy, we repeat 50 trials to obtain stable results.}}
% \label{tab:schedule_metric_choice}
% \end{table*} 


    


    % \begin{figure*}[ht]
    %     \centering
    %     \begin{subfigure}[b]{0.475\textwidth}
    %         \centering
    %         \includegraphics[width=\textwidth]{imgs/candidate_selection/cifar10-madry/targeted/modelB_D_E.png}
    %         \caption[]%
    %         {Local Model: Model A Model B Model C}    
    %         \label{fig:candi_selection_robust_tar_cifar10_modelb_d_e}
    %     \end{subfigure}
    %     \hfill
    %     \begin{subfigure}[b]{0.475\textwidth}  
    %         \centering 
    %         \includegraphics[width=\textwidth]{imgs/candidate_selection/cifar10-madry/targeted/densenet_resnet_E.png}
    %         \caption[]%
    %         {Local Model: Adv-DenseNet Adv-ResNet Model C}    
    %         \label{fig:candi_selection_robust_tar_cifar10_dense_b_d}
    %     \end{subfigure}
    %     \hfill
    %     \begin{subfigure}[b]{0.475\textwidth}  
    %         \centering 
    %         \includegraphics[width=\textwidth]{imgs/candidate_selection/cifar10-madry/targeted/densenet_resnet_B.png}
    %         \caption[]%
    %         {Local Model: Adv-DenseNet Adv-ResNet Model A}    
    %         \label{fig:candi_selection_robust_tar_cifar10_dense_resnet_b}
    %     \end{subfigure}
    %     \hfill
    %     \begin{subfigure}[b]{0.475\textwidth}  
    %         \centering 
    %         \includegraphics[width=\textwidth]{imgs/candidate_selection/cifar10-madry/targeted/densenet_resnet.png}
    %         \caption[]%
    %         {Local Model: Adv-DenseNet Adv-ResNet}    
    %         \label{fig:candi_selection_robust_tar_cifar10_dense_resnet_vgg}
    %     \end{subfigure}
    %     \vskip\baselineskip
    %     \caption[]
    %      {Targeted Attack on Robust CIFAR10 Model: Candidate Transfer Rate with Respect to Candidate Rate} 
    %     \label{fig:candi_selection_robust_tar_cifar10}
    % \end{figure*}


%As shown in Figure \ref{fig:metric_choice}, seed prioritization strategies based on attack loss (i.e., Vanila-Attack-Loss, PGD-Step+Attack Loss) have closest performance to the retroactive optimal one and outperforms the random scheduling strategy significantly. To demonstrate the optimized effect of PGD Step + Attack Loss over Vanila-Attack-Loss strategy in the initial query step, we show zoom-in version of Figure \ref{fig:metric_choice_sub} on its right-hand side. 

%More quantitative information is provided in Table \ref{tab:schedule_metric_choice}, where we record the queries needed to successfully attack one, top 1\%, top 2\%, top 5\% and 10\% of the total candidate seeds (1000 images). We observe that for finding the first adversarial example, the retroactive optimal strategy only takes 1 query while PGD Step + Attack Loss strategy takes 3 queries. In contrast, with random scheduling or scheduling purely based on PGD Steps, the number of needed queries are 293 and 530 respectively. The performance gain of PGD Step + Attack Loss or Vanila-Attack Loss get larger as number of attacked seeds increases. For example, when attacker is interested in 5\% of the total 1000 candidate seeds, with PGD Step + Attack Loss strategy, it only costs 1/515 of the queries of random scheduling strategy. Therefore, we demonstrate that, there exists efficient and effective strategy to identify easy-to-attack seeds in early stage and can save the query efficiency significantly in query limited batch setting. Since attack loss based strategy provides best scheduling performance, in next section, we only consider adopting PGD Step + Attack Loss strategy. 


   

 
% \begin{table*}[tbh]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
% Attack Method & Model & Attack & First AE & 1\% & 2\% & 5\% & 10\% \\ \hline
% \multirow{4}{*}{AutoZOOM} & \multirow{2}{*}{MNIST Normal} & Local Adv & 2 & 11 & 21 & 51 & 101 \\ \cline{3-8} 
%  &  & Orig Seed & 3 & 2,401 & 6,773 & 17,159 & 51,857 \\ \cline{2-8} 
%  & \multirow{2}{*}{CIFAR10 Robust} & Local Adv & 2 & 11 & 21 & 51 & 210 \\ \cline{3-8} 
%  &  & Orig Seed & 3 & 65 & 145 & 739 & 2,521 \\ \hline
% \end{tabular}
% \caption{Comparison of Different Batch Attack Strategies: \footnotesize{``First AE" and columns of ``x\%" denotes the number of queries needed to find x\% fraction of adversarial examples out of the total candidate seeds. Two attacks that start from original seed and local adversarial example both adopt greedy seed prioritization strategy based on attack loss.}}
% \label{tab:hybrid_batch_eval}
% \end{table*}

% \begin{table*}[tbh]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
% Attack & Start Point & Local Model & First AE & 1\% & 2\% & 5\% & 10\% \\ \hline
% \multirow{3}{*}{NES} & \multirow{2}{*}{Local Adv} & All Robust & 1 & 12 & 25 & 64 & 120 \\ \cline{3-8} 
%  &  & All Normal & 1 & 20 & 63 & 261 & 1,505 \\ \cline{2-8} 
%  & Orig Seed & - & 51 & 510 & 1,370 & 5,850 & 19,700 \\ \hline
% \multirow{3}{*}{AutoZOOM} & \multirow{2}{*}{Local Adv} & All Robust & 1 & 12 & 25 & 64 & 120 \\ \cline{3-8} 
%  &  & All Normal & 1 & 20 & 63 & 261 & 1,086 \\ \cline{2-8} 
%  & Orig Seed & - & 3 & 100 & 216 & 800 & 2,618 \\ \hline
% \end{tabular}
% \caption{Untargeted attack on robust CIFAR10 model: comparison of hybrid attack to baseline attack in batch setting \footnotesize{ ``All Normal" denotes local ensemble of (ModelA, ModelB, ModelC). ``All Robust" denotes local ensemble of (Adv-DenseNet, Adv-ResNet). ``First AE" and columns of ``x\%" denotes the number of queries needed to find x\% fraction of adversarial examples out of the total candidate seeds.}}
% \label{tab:hybrid_batch_eval}
% \end{table*}


%\color{blue}{\subsection{Hybrid Batch Attacks}\label{sec:hybrid_batch_eval}
%Similarly, our hybrid attack strategy comes with seed prioritization strategy based attack loss (PGD-Step+Attack-Loss). 


%\snote{did not modify the content of this section much. Basically, here I am choosing the best performing two-stage strategy on hybrid attack and target loss based two-stage strategy (in the first stage, images can only be queried in random order because no local info is available) when attacks start from original seed. It is very important to note that, when attacks start from original seed, there is no local model info available. Therefore, except for prioritizing based on target loss, there are no ways to prioritize seeds. Therefore, attackers can still benefit by first querying some seeds and then attack the seeds in the sorted order based on target loss. Comparisons in Figure 5 might not be the most fair comparison. Will address it when other parts are all set. }
%In this section, we evaluate the performance gain of hybrid attacks in the batch setting. We use the same gradient based attacks -- AutoZOOM and NES. The baseline method is execution of the gradient attack from original seed while the hybrid attack starts from the local AEs. We demonstrate in this section that, hybrid attack strategy also improves query efficiency significantly in query limited setting. 

%We first provide details on the seed prioritized baseline method: the baseline method does not have access to any local model information to prioritized the ``easy-to-attack" seeds. The only information that can be utilized to sort the seeds is to query each seed once to get the target model prediction score and leverage target loss value to identify easy seeds. Our experimental results indicate that with prioritization based on target loss value, baseline method can also be made much more query efficient compared to the random strategy of the baseline method and has closer performance to the retroactive optimal strategy of the baseline method. We further assume the baseline method can obtain the target model prediction score for free and therefore can prioritize seeds with target loss value without any overhead, which is actually an upper bound for the greedy strategy of baseline methods \footnote{We take this upper bound as our baseline strategy because, without the assumption of free access to initial target model prediction score, querying all seeds once to obtain the target loss value may no longer be the optimal choice. Attackers may benefit more by querying some seeds once and start to attack the queried seeds in the sorted order. For simplicity, we assume attacker has free access to target loss value and therefore, is always the optimal choice for attacker to attack in the sorted order based on target loss value.}. 

%Figure \ref{fig:performance_comparison} provides the evaluation results on CIFAR10 robust model, with local models being all normal and all robust. We choose CIFAR10 robust model as it is the hardest scenario for hybrid batch attacks. It is obvious that hybrid attack still has significantly better performance in finding more number of adversarial samples, compared to the baseline attack under the same query limit. In Table \ref{tab:hybrid_batch_eval}, we provide more quantitative information regarding Figure \ref{fig:performance_comparison}. Specifically, for untargeted NES attack on robust CIFAR10 model with all robust local models, the seed prioritized hybrid attack strategy finds 1\% of adversarial example in 12 queries while baseline strategy requires 510 queries: the hybrid attack strategy only consumes approximately 1/50 of queries of the baseline attack. In table \ref{tab:hypo_loc_adv_sample}, we show that with all normal local models, the performance gain of hybrid attack is not significant compared to starting from original seeds. However, in batch attack setting, attacker can still obtain significant query savings by adopting the hybrid strategy. For example, when the attacker is interested in obtaining 10\% of the total seeds, for untargeted AutoZOOM attack with all normal local models, the hybrid attack strategy only takes lower than 1/2 of queries of the baseline method (1,086 queries for hybrid attack strategy and 2,618 for the baseline attack strategy). 
%Results of other attack and other models show similar performance and the least significant performance gain is actually observed on hybrid attack for CIFAR10 robust models, which, as demonstrated, still saves query efficiency significantly.  
%}

% In this section, we provide detailed performance analysis of hybrid attacks with different attacker knowledge in terms of local models. Specifically, the attacker either has access to well-trained local models or just models with random initialization. Models with random initialization are more challenging tasks as the attacker does not have proper access to standard training data of the target model. We name the hybrid attack as \textbf{attack 1}.
% \subsection{Hybrid Attack with Pretrained Models}\label{subsec:pretrained_model}
% In this section, we analyze the performance of hybrid attack in batch setting, when the attacker has access to several pretrained local models.\\
% \textbf{Note: in this mode, for MNIST, CIFAR10, experimental results all show that it can improve significantly compared to current standard attacks. I will present results based on the frequency of the sub model fine-tuning process. If the frequency is set to be the length of the total pool of seeds, then there is no substitute model training required} 


% % \subsubsection{Hybrid Attack with Local Model Fine-Tuning}
% % In this attack mode, attacker follows the attack procedure outlined in Algorithm \ref{alg:hybrid} and fine-tunes the pretrained local models with the outputs from gradient estimation based attacks. \\

% % \subsubsection{Hybrid Attack with Local Model Fine-Tuning}
% % In this attack mode, attacker no longer fine-tunes the local models, instead directly takes the locally generated adversarial samples as the starting points for the gradient estimation based attacks. We name the hybrid attack as \textbf{attack 1.2} 

% \subsection{Hybrid Attack with Random Models}\label{subsec:random_model}
% In this section, we analyze the performance of hybrid attack in batch setting, when the attacker has access to randomly initialized local models.  We name the hybrid attack as \textbf{attack 2} \\
% \textbf{Note: in this mode, for MNIST, it can improve significantly compared to current standard attacks. For CIFAR10, I am unable to obtain reliable models and transfer rate is very low. Therefore, the possible explanation is that CIFAR10 is way more complex and unable to learn meaningful classifiers only based on ZOO attack outputs.}

% \subsection{Comparisons of Different Hybrid Attack Forms}
% In this section, we provide experimental results of different hybrid attack forms discussed in section \ref{subsec:pretrained_model} and section \ref{subsec:random_model}.\\ 
% \textbf{Note: In this section, experimental results for MNIST show that fine-tuning local models gives better results. For CIFAR10, hybrid attack without local model fine-tuning gives best performance. Possible explanation here is that, CIFAR10 is still more complex and cannot shape better models with ZOO attack results}

